An Addendum to NeBula: Towards Extending TEAM CoSTAR's Solution to Larger Scale Environments

This paper presents an appendix to the original NeBula autonomy solution developed by the TEAM CoSTAR (Collaborative SubTerranean Autonomous Robots), participating in the DARPA Subterranean Challenge. Specifically, this paper presents extensions to NeBula's hardware, software, and algorithmic components that focus on increasing the range and scale of the exploration environment. From the algorithmic perspective, we discuss the following extensions to the original NeBula framework: (i) large-scale geometric and semantic environment mapping; (ii) an adaptive positioning system; (iii) probabilistic traversability analysis and local planning; (iv) large-scale POMDP-based global motion planning and exploration behavior; (v) large-scale networking and decentralized reasoning; (vi) communication-aware mission planning; and (vii) multi-modal ground-aerial exploration solutions. We demonstrate the application and deployment of the presented systems and solutions in various large-scale underground environments, including limestone mine exploration scenarios as well as deployment in the DARPA Subterranean challenge.

==> template_files/instructions.tex <==
\section*{\comb{ {\bf @CoSTARs}: Please have a look at the following formatting instructions}}
\comb{
\subsection{General formatting instructions}
\label{gen_inst}

The main text of your paper should be in a single column textbox 6.5
inches by 9 inches. Regular text should be in a 12 point font.
Paragraphs should not be indented, and should be separated by a
single line space.

Please pay attention to the instructions in the next section 
regarding figures, tables, acknowledgments, and references.

\subsubsection{Formulation}

I've added the mathsym.tex file to standardize the addition of formulas. I suggest to use the following:
\begin{equation}
\begin{split}
    \bfM: Matrix \\
    \bfv: Vector \\
    s: Scalar    
\end{split}
\end{equation}

Please, when adding your stuff, try to follow some standards so it'll be easier later on.

\subsubsection{Citations within the text}

Citations should follow the APA style \cite{apa}. Unlike many
scientific papers, this requires in text citation of authors' names
and date of work. The corresponding references are to be listed in
alphabetical order using APA reference style at the end of the
paper, in the \textbf{References} section. Example references are
given in this template for books with one author \cite{baxter},
conference papers \cite{binh}, journal articles \cite{baldwin}, and
books with editors \cite{stock}. For electronic references without
authors, the reference is cited using the web page title. The
University of Wisconsin Writing Center provides a good resource for
questions about the APA style \cite{wisconsin}.

\subsubsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first
footnote} in the text. Place the footnotes at the bottom of the page
on which they appear. Precede the footnote with a horizontal rule of
2~inches.\footnote{Sample of the second footnote}

\subsubsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. We recommend using either the jpg or the embedded
postscript format for images and the tiff format for line drawings.
If the figures contain graphs, please ensure that the axis labels
are legible when printed. Figure number and caption always appear
after the figure. Place one line space before the figure caption,
and one line space after the figure. The figure caption is lower
case (except for first word and proper nouns); figures are numbered
consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

\begin{figure} [h]
    \centering
    \includegraphics[height=2.0in]{figures/g1}
    \hspace{.2in}
    \includegraphics[height=2.0in]{figures/g2}
    \caption{Line graph of random numbers (left) and bar graph of random numbers (right)}
    \label{fig:sampleFigure}
\end{figure}

\subsubsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. Table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title} \label{sample-table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
% after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
   & $k_{g}$ & $k_{o}$ & $c_{3}$ & $c_{4}$ & $c_{5}$ \\
  \hline\hline
  Careful/Sparse & 0.334 & 0.597 & 1.101 & 9.621 & 8.170 \\ \hline
  Careful/Dense & 3.124 & 3.195 & 1.094 & 5.899 & 7.318 \\ \hline
  Aggressive/Sparse & 0.840 & 9.153 & 2.853 & 8.274 & 0.187 \\ \hline
  Aggressive/Dense & 4.838 & 2.841 & 0.670 & 7.952 & 0.386 \\ \hline
  Hand-Tuned & 0.767 & 0.060 & 0.340 & 2.000 & 0.250 \\
  \hline
\end{tabular}
\end{center}
\end{table}

\subsubsection{APA Reference Style}

References follow the acknowledgments. Use an unnumbered third level
heading for the references. References must be listed in the APA
format (available at http://www.apastyle.org/). References should be
in the same font size as the paper text.


} % end of comb
